Search for a Higgs boson decaying to massive vector boson pairs at LEP

This dissertation presents a search for a Higgs boson decaying to massive vector boson pairs. The search is based on data collected by the L3 experiment at CERN during the 1999-2000 period. We present the details and results of analyses for six of the physical channels of hZ->WWff. The combined analyses exclude a fermiophobic Higgs decaying to massive vector boson pairs for 83.8 GeV < m_h < 104.2 GeV at a 95% confidence level with an unexcluded region between 88.8 GeV < m_h < 89.6 GeV. Monte Carlo predictions of the analyses' performance predict an exclusion range of 86.8 GeV < m_h <107.5 GeV. We also present model-independent branching ratio limits for the massive vector boson search, as well as a scan of the fermiophobic plane combining with the results of the LEP h->gamma gamma search.

==> junk/q.tex <==
\relax 
\@setckpt{text/intro}{
\setcounter{page}{3}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{r@tfl@t}{0}
}

